BoundED: Neural Boundary and Edge Detection in 3D Point Clouds via Local Neighborhood Statistics

Extracting high-level structural information from 3D point clouds is challenging but essential for tasks like urban planning or autonomous driving requiring an advanced understanding of the scene at hand. Existing approaches are still not able to produce high-quality results consistently while being fast enough to be deployed in scenarios requiring interactivity. We propose to utilize a novel set of features describing the local neighborhood on a per-point basis via first and second order statistics as input for a simple and compact classification network to distinguish between non-edge, sharp-edge, and boundary points in the given data. Leveraging this feature embedding enables our algorithm to outperform the state-of-the-art techniques in terms of quality and processing time.

==> tex/graphical_abstract.tex <==

%%Graphical abstract
\begin{graphicalabstract}
    \fbox{\includegraphics[width=13cm]{additional_documents/graphical_abstract/graphical_abstract.pdf}}
    \vfill
\end{graphicalabstract}

==> tex/research_highlights.tex <==

\begin{highlights}
    \item Edge and boundary detection in 3D point clouds is important for scene understanding
    \item We present a novel feature embedding for local point neighborhoods
    \item An MLP is used to classify sharp-edge and boundary points based on the embedding
    \item Evaluation on synthetic point clouds and on scans of real-world buildings and plants
    \vfill
\end{highlights}
